Toward Physics-guided Time Series Embedding

In various scientific and engineering fields, the primary research areas have revolved around physics-based dynamical systems modeling and data-driven time series analysis. According to the embedding theory, dynamical systems and time series can be mutually transformed using observation functions and physical reconstruction techniques. Based on this, we propose Embedding Duality Theory, where the parameterized embedding layer essentially provides a linear estimation of the non-linear time series dynamics. This theory enables us to bypass the parameterized embedding layer and directly employ physical reconstruction techniques to acquire a data embedding representation. Utilizing physical priors results in a 10X reduction in parameters, a 3X increase in speed, and maximum performance boosts of 18% in expert, 22% in few-shot, and 53\% in zero-shot tasks without any hyper-parameter tuning. All methods are encapsulated as a plug-and-play module

==> structure/1_intro_0.tex <==
\section{Introduction}
\label{sec:intro}

\begin{wrapfigure}{r}{0.382\textwidth}
\label{fig:radar}
  \begin{center}
  \vspace{-17pt}
    \includegraphics[width=0.382\textwidth]{fig/radar.png}
  \end{center}
  \vspace{-13pt}
  \caption{\small{Performance comparison of physics-guided time series embedding versus original method across eight aspects.}}
  \vspace{-14pt}
\end{wrapfigure}
 


The explosion of real-time sensing data from the physical world opens up new opportunities for data-driven decision-making \citep{yu2024learning}. In numerous scientific and engineering disciplines, a central focus lies in dynamical systems that evolve over space and time, exampled in fluid mechanics, thermodynamics, asymptotic dynamics, and neuroscience \citep{brunton2020machine,tan2023selecting,chen2021high}. With the emergence of massive data, data-driven time series analysis has achieved success in energy, transportation, meteorology, and other domains by leveraging the strong fitting capabilities of neural networks for real-world data \citep{wu2021autoformer,nie2022time,hu2024time}. According to the Takens \citep{takens2006detecting} and Whitney theorems \citep{whitney1936differentiable}, time series can be viewed as observations stemming from underlying dynamical systems. However, these two fields of research continue to remain disparate.

As illustrated in Figure \ref{fig:overall}, dynamical systems are defined by coupled differential equations that describe the evolution of spatial coordinates over time. Typically, the analytic solution is not numerically feasible, and current efforts primarily integrate boundary constraints or real-value corrections to study the evolution patterns of the systems, thus requiring strong modeling assumptions and being computationally expensive.

These models are derived from first principles, can guarantee conservation laws, and are easy to interpret.
Yet, physics-based approaches require strong modeling assumptions and manually crafted features and are typically computationally expensive. It is hard to simplify the model while maintaining satisfactory accuracy. For real-world systems with unknown dynamics, the strong assumptions in physics-based approaches can easily break down.
Our main goal is to develop a rich body of empirical and theoretical connections between physics-driven dynamical system modeling and data-driven time series analysis. One of the most notable differences lies in XXX, as depicted in Figure 2, where dynamical system modeling XXX, its advantages XXX, and disadvantages XXX, while time series analysis XXX, its advantages XXX, and disadvantages XXX. To address this, we focus on the initial stage XXX and propose physics-guided time series embedding, with its advantages XXX. As illustrated in Figure 1, we have enhanced the performance of various model architectures on real-time series analysis benchmarks. As immediate consequences of this paper:

\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=0pt]
  \item We innovatively integrate dynamical system embedding theory into the Time Series Analysis tasks, bridging physical-guided embedding and parameterized embedding from both empirical and theoretical perspectives. \textbf{\textit{Embedding Duality}} and \textbf{\textit{Dim Scaling Law}} are proposed.
  % \item For expert models, employing physical-guided embedding results in a maximum \textbf{\textit{10$\times$ reduction in parameter}}, a \textbf{\textit{3$\times$ increase in speed}}, \textbf{\textit{enhanced gradient stability}}, and \textbf{\textit{improved performance}} across all four types of Time Series Analysis tasks and all four neural network architectures.
  \item For expert tasks, we comprehensively investigated the performance differences over \textbf{\textit{12 embedding techniques}}, with physical-guided embedding results in a maximum \textbf{\textit{10$\times$ reduction in parameter}}, a \textbf{\textit{3$\times$ increase in speed}}, \textbf{\textit{enhanced gradient stability}}, and \textbf{\textit{improved performance}} across all four types of Time Series Analysis tasks and all four neural network architectures. The efficiency will significantly enhance various real-world applications and deployment.
  \item For foundation tasks, the utilization of physical-guided embedding remains \textbf{\textit{in line with Scaling Laws}}. Additionally, the generalization properties of dynamical system topologies lead to maximum performance enhancements of \textbf{\textit{38\% in zero-shot}} and \textbf{\textit{27\% in few-shot}} tasks. The generalization is expected to foster the emergence of physical-guided time series foundation models.
\end{itemize}




\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{fig/overall.png}
    \caption{Dynamical systems embody physical laws unfolding in space and time, with time series as the low-dimensional observations. Our embedding duality theory bridges these two frameworks, demonstrating that parameterized hidden state representations are the model's estimation of dynamical system structures.}
\label{fig:overall}
\vspace{-1.5em}
\end{figure}








==> structure/2_background_0.tex <==
\vspace{-0.5em}
\section{Formulation}
\vspace{-0.5em}
\label{sec:background}


\begin{definition}[\textbf{Dynamical System}]
% \small
    Let the domain $S$ be an open subset of $\mathbbm{R}^d$ and set an integer $k \geq 1$. Define the system state as $\boldsymbol{x}: S \mapsto \mathbbm{R}^m$ where $\boldsymbol{x}=\left(x^1, \ldots, x^m\right)$. Then, an expression of:
$$
\mathcal{F}\left(D^k \boldsymbol{x}(s), D^{k-1} \boldsymbol{x}(s), \ldots, D \boldsymbol{x}(s), \boldsymbol{x}(s), s\right)=0
$$
is called a $k^{\text {th}}$ order system of partial differential equation (or ordinary differential equation when $d=1$), where $\mathcal{F}: \mathbbm{R}^{m d^k} \times \mathbbm{R}^{m d^{k-1}} \times \ldots \times \mathbbm{R}^{m d} \times \mathbbm{R}^m \times S \mapsto \mathbbm{R}^m$ and $s \in S$.

In some dynamical systems literature \citep{hu2024attractor,de2023time,vlachos2008state}, continuous dynamical systems are defined on locally differentiable manifold spaces $\mathcal{M}$, where $\mathbbm{R}$ in Definition \ref{def:DS} can be viewed as discrete records of the continuous state.

\label{def:DS}
\normalsize
\end{definition}

\begin{formulation}
For standard time series analysis tasks, with historical sampled data $\bm{U}\in\mathbb{R}^{C \times T}$, we aim to derive a nonlinear mapping ${f}:\bm{U}\rightarrow\bm{Y}$ for predicting future values over $H$ time steps. Within the physics-guided framework, at each time step t, ${f}$ can be decomposed into:

(1) $\operatorname{Rec}_t$ employs mathematical methods to reconstruct the underlying dynamical system based on time series data $\bm{U}$, \faSearch ~\underline{which is the research focus of this paper presented in Section \ref{sec:physics-guided emb}}.

(2) $\operatorname{Evo}_t$ serves as arbitrary neural networks to parameterize system evolution within Sobolev space, which is selected as four different model backbones detailed in Appendix \ref{apx:encoders}.
\normalsize
\end{formulation}

\vspace{-0.5em}
\section{Related Work}
\vspace{-0.5em}
\noindent \textbf{Parameterized Embedding in Deep Time Series Models}.~
% \paragraph{Parameterized Embedding in Deep Time Series Analysis.}
The embedding technique, serving as a space transformation $\mathbbm{R}^n \mapsto \mathbbm{R}^m$, facilitates the mapping of discrete sparse features into continuous dense vector representations, laying a solid foundation for success across various machine learning domains. In time series analysis benchmark, mainstream methods utilize patch operation (Figure \ref{fig:embeddings}a) to conduct local linear projection \citep{nie2022time}, with certain models using convolutions to address inter-block information isolation \citep{hu2024twins,zhang2024multi,lin2024sparsetsf}. Additionally, for audio modeling tasks, windowed spectral transformation techniques (Figure \ref{fig:embeddings}b), such as the short-time Fourier transform, are commonly employed to extract time-frequency representations, thereby addressing concerns related to information density \citep{erol2024audio}. Grid embeddings (Figure \ref{fig:embeddings}c) are commonly employed to handle the spatial-temporal relationships within the data \citep{gupta2021multiwavelet,wu2023solving}. Furthermore, several studies leveraged self-supervised learning to obtain enhanced embedding representations \citep{lee2023learning,fraikin2023t}.
% [connection] However, these parameterized XXXX

\noindent \textbf{Embedding Theory for Dynamics System Reconstruction.}.~
% \paragraph{Embedding Theory for Dynamics System Reconstruction.}
% Dynamical systems are typically defined by coupled differential equations that describe the evolution of spatial coordinates over time.
Since significant results proposed by \citep{whitney1936differentiable,takens2006detecting} and formalized in \citep{sauer1991embedology}, the Embedding Theory has pervaded through almost all aspects of nonlinear dynamical systems (Definition \ref{def:DS}). The time series $x(t)\in\mathbbm{R}^{n}$ can be broadly interpreted as successive, though not always regular, observations of a dynamic system $\mathcal{F}\in\mathbbm{R}^{m}$ via a measurement function $h: \mathbbm{R}^{m} \mapsto \mathbbm{R}^{n} (n\textless m)$. The main goal is to reconstruct the underlying system and explore its properties, which paved the way for developing numerous techniques like derivatives \citep{packard1980geometry}, integrals \citep{RevModPhys.70.1455}, time delay \citep{takens2006detecting, abarbanel1994predicting}, and principal component embedding \citep{broomhead1986extracting}. The system dynamics is subsequently learned using preferred modeling tools such as recurrent neural networks \citep{sangiorgio2020robustness}, state space models \citep{alonso2024state, hu2024attractor}, and reservoir computing \citep{haluszczynski2019good,yan2024emerging}, etc. Attraos \citep{hu2024attractor} pioneered using the time delay embedding technique in time series forecasting tasks, while our paper extensively explores various embedding techniques in Section \ref{sec:physics-guided emb}.




% \begin{remark}
% % \small
%     In some dynamical systems literature \citep{hu2024attractor,de2023time,vlachos2008state}, continuous dynamical systems are defined on locally differentiable manifold spaces $\mathcal{M}$, where $\mathbbm{R}$ in Definition \ref{def:DS} can be viewed as discrete records of the continuous state.
% \normalsize
% \end{remark}












==> structure/3_architecture_0.tex <==
\vspace{-1em}
\section{Physics-guided Time Series Embedding}
\vspace{-1em}
\label{sec:physics-guided emb}

% In this section, we commence by elucidating the implementation details and characteristics of our proposed physic-guided embedding techniques summarized in Table \ref{tab:various embs}, progressing to the Embedding Duality Theory. All the proofs in this paper can be found in Appendix \ref{sec:proof}.
In this section, we commence by elucidating the implementation of physic-guided embeddings summarized in Table \ref{tab:various embs}, progressing to the Embedding Duality theory. Proofs are in Appendix \ref{sec:proof}.

\begin{figure}
    \centering
    \vspace{-0.5em}
    \hspace*{-0.5ex}
    \begin{adjustbox}{width=1.03\columnwidth, center}
    \includegraphics[width=1.\columnwidth]{fig/Embs3.png}
    \end{adjustbox}
    \caption{Existing parameterized embedding (a-c) and physics-guided non-parametric embedding (d-f) techniques. 
(a) Each time series patch utilizes a shared linear projection layer to obtain hidden representations.
(b) Dense time series are processed using windowed spectral transformations with gradients for adaptability.
(c) Multivariant time series are embedded using a shared linear layer on a grid measure.
(d) Time Delay embedding based on predetermined hyper-parameters.
(e) Higher-order derivative values are concatenated to reconstruct dynamic structures.
(f) Integral terms can replace higher-order derivatives to address numerical instability.
}
\label{fig:embeddings}
\vspace{-1.5em}
\end{figure}

% \small
% \begin{definition}[\color{blue}Problem Setting]
% For standard time series analysis tasks, with historical sampled data $\bm{U}\in\mathbb{R}^{C \times T}$, we aim to derive a nonlinear mapping ${f}:\bm{U}\rightarrow\bm{Y}$ for predicting future values over $H$ time steps. Within the physics-guided framework, ${f}$ can be decomposed into the dynamical system reconstruction operator $\operatorname{Rec}_t$ and evolution operator $\operatorname{Evo}_t$ at every time t, with following properties:

% (1) $\operatorname{Rec}_t$ employs mathematical methods to reconstruct the underlying dynamical system based on time series $\bm{U}$, utilizing it as the initial representation of the data.

% (2) $\operatorname{Evo}_t$, serving as an arbitrary neural network architecture, is utilized to parameterize the evolution of function-to-function dynamical systems within the Sobolev space.
% \normalsize
% \end{definition}
\vspace{-0.5em}
\subsection{Technical Details}
\vspace{-0.5em}
\paragraph{Time Delay Embedding (TD-Emb).}
In Equation \ref{eq:time-delay}, time delay embedding involves the augmentation of scalar time series ${x}(t)$ into a higher-dimensional dynamical system $\vec{x}(t)$ by two hyper-parameters, namely, embedding dimension $m$ and time delay $\tau$ (Figure \ref{fig:overall}d). 
% Theoretically, when $m > 2n+1$, it is possible to perfectly reconstruct the dynamical structures \citep{vlachos2008state}. 
To simplify the method, $\tau$ is set heuristically as a quarter of the most dominant period in the signal\footnote{The sine wave ${x}(t)=\sin(\omega t)$ yields the most circular embedding in a 2D plane with $\tau=2\pi/4\omega$} and $m$ is determined by the CC method \citep{kim1999nonlinear}. For multivariate time series analysis, we can either employ a channel-independent strategy (CI) or concatenate $\{\vec{x}_i(t)\}_{i=1}^C$ \citep{vlachos2008state} to construct a unified system (CD). Furthermore, we segment the dynamical representation to enhance model stability and reduce computational complexity, which will be omitted in the subsequent description.
\begin{equation}
% \vec{x}(t)=(x(t), x(t-\tau), \ldots, x(t-(m-1) \tau)), \quad \quad \quad \vec{x}(t)_{patch} = \operatorname{Unfold}~(\operatorname{Pad}(\vec{x}(t)), p, s).\footnote{Experimental results indicate that zero-padding on the left side of $\vec{x}(t)$ achieves optimal performance.}
\vec{x}(t)=(x(t), x(t-\tau), \ldots, x(t-(m-1) \tau)), \quad \quad \quad \vec{x}(t)_{patch} = \operatorname{Unfold}~(\operatorname{Pad}(\vec{x}(t)), p, s).
\label{eq:time-delay}
\end{equation}
% \begin{remark}
%     Time delay embedding stands as the only method enabling visualization of dynamical structures within Euclidean space, but hyper-parameters $m$ and $\tau$ significantly impact performance. The Principal Component embedding builds upon time delay embedding, detailed in Appendix \ref{bg:pca emb}.
% \end{remark}
Time delay embedding stands as the only method enabling visualization of dynamical structures within Euclidean space, but hyper-parameters $m$ and $\tau$ significantly impact performance. The Principal Component embedding builds upon time delay embedding, detailed in Appendix \ref{bg:pca emb}.
\begin{remark}
    For multivariate series, the choice between CI and CD modeling strategies should be guided by the mutual information and Lyapunov exponents of the variables, detailed in Appendix \ref{apx:exp}.
\end{remark}
\begin{remark}
    Experimental results indicate that zero-padding on the left side of $\vec{x}(t)$ achieves optimal performance compared to left repetition, right repetition, and right zero-padding.
\end{remark}

\vspace{-1em}
\paragraph{High-order Derivatives Embedding (HD-Emb).} Based on the multi-order characteristics of the dynamical system in Definition \ref{def:DS}, a straightforward approach is to employ high-order derivatives to reconstruct the dynamic structure. In practical applications, we utilize the Forward Differencing (Equation \ref{eq:differencing}) to simulate the process of continuous derivatives (Equation \ref{eq:derivates}) with hyper-parameter $m$ and $\Delta$.

% \small
% \vspace{-0.25em}
\begin{minipage}{.5\linewidth}%
\begin{equation}
\vec{x}(t)=\left(x(t), \frac{d x(t)}{d t}, \ldots, \frac{d^m x(t)}{d t^m}\right),
\label{eq:derivates}
\end{equation}
\end{minipage}
\begin{minipage}{.5\linewidth}%
\begin{equation}
\frac{d x(t)}{d t} \approx \frac{x(t+\Delta)-x(t)}{\Delta}.
\label{eq:differencing}
\end{equation}
\end{minipage}
\normalsize
% \begin{proposition}
% Existing neural network architectures all resemble the learnable differential process.
% \end{proposition}

Although $m$ and $\Delta$ can still be calculated using numerical methods \citep{tan2023selecting}, experiment results indicate that $m=3$ and $\Delta=1$ generally yield the best performance. In some studies related to ordinary differential equations and state-space models \citep{smith2022simplified,gu2023mamba,hu2024time}, $\Delta$ is defined as a learnable parameter to selectively emphasize important information in the data. In this research, we prioritize the efficiency of non-parameterized physical priors, while the exploration of trainable High-order Derivatives embedding is left for future work.

\vspace{-0.5em}
\paragraph{Integral-differential Embedding (ID-Emb)).} Approximations of successive higher-order derivatives are generally inaccurate as the signal-to-noise ratio tends to be negatively impacted. An alternative method is integral-differential embedding (Equation \ref{eq:indiff}) with only hyper-parameter $\Delta$.
% \vspace{-0.5em}
\begin{equation}
\vec{x}(t)=\left(\int_{-\infty}^t x(t) d t, x(t), \frac{d x(t)}{d t}\right), \quad \quad \quad \quad \quad \int_{-\infty}^t x(t) d t \approx \Delta \sum_{i=1}^{T}x(t+i\Delta).
\label{eq:indiff}
\end{equation}
In this approach, the hidden-state dimension is constrained to 3. While this optimizes efficiency, the expressive capacity of model is constrained. As shown in Table \ref{tab:various embs}, experiment results reveal that ID-Emb consistently underperforms TD-Emb and HD-Emb methods. Therefore, in the experimental section, we focus primarily on investigating the improvements brought by these two approaches.

\begin{remark}
    We have encapsulated various embedding methodologies and their associated encoder \& decoder modules in the code repository, facilitating direct invocation with \textbf{a single line of code}.
\end{remark}

\begin{table}
% \small
\vspace{-0.5em}
        \centering
	\caption{Comprehension comparison for various physics-guided embedding methods}
 \vspace{-0.5em}
 \renewcommand{\arraystretch}{0.9} 
        \setlength{\tabcolsep}{10pt}
        \begin{adjustbox}{width=1\columnwidth, center}
        \resizebox{1\columnwidth}{!}{
        \begin{tabular}{c|c|c|c|c|c}
\toprule
Method & Interpretability & Performance & Robustness & Convergence Rate & Hyper-parameter \\ 
\midrule
\textbf{TD-Emb} & $1^{st}$ & $2^{nd}$ & $3^{rd}$ & $1^{st}$ & $m,\tau\leftarrow$ physical prior \\
\midrule
\textbf{HD-Emb} & $2^{nd}$ & $1^{st}$ & $1^{st}$ & $3^{rd}$ &  $m,\Delta\leftarrow$ typically (3,1) \\
\midrule
\textbf{ID-Emb} & $3^{rd}$ & $3^{rd}$ & $2^{nd}$ & $2^{nd}$ & $\Delta\leftarrow$ typically (1) \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-1.5em}
\label{tab:various embs}
\end{table}

\vspace{-1em}
\subsection{Theoretical Justification for Embedding Duality}
\label{sec:emb duality}
\vspace{-0.25em}
% 首先patch操作可以视为一种积分变换，进行空间变换，投影到谱空间
% patch序列满足W^-1AW的动力学。
%% (由于激活函数导致Liptiz连续)梯度即雅可比 + 伪动力结构 --> 空间放缩 + 初始球面 + SVD分解 --> 椭球   
% 嵌入矩阵相当于非线性动力的线性化，给时间序列赋予动力学梯度,随着patch_len逐渐增大，将舍弃更多的非线性特征？
% encoder是1-liptiz，则不会影响到动力结构的改变


% 首先patch是一种积分变换，将时间序列投影到谱空间用于建模时间序列动力学
% 其次给定原始动力学f，在谱空间中patch序列的动力学为WJW, 可视为约旦标准型
% 接下来我们将关注训练过程中动力系统结构的变化
% Liptiz代表随扰动，函数的变化率，lemma3说明encoder不会破坏使得我们可以忽略encoder的影响只关注embedding部分的变化，同时我们认为卷积ssm是更适合建模时间序列的架构，而标准trans，梯度将会引发动力结构剧烈变化，从而破坏原始动力学特征。
% 在训练过程中，embedding的损失会影响到J，从而使得特征空间收缩，如图X，XXX，然而缺乏物理约束经常过拟合，并且梯度震荡现象。
% 同时在嵌入理论中，动力结构会随嵌入空间的变化而发生结构变化，过小XXX，过大会稀疏并且放大噪声的影响，通常这个阈值2，当超过潜在2倍维度，被称为寄生相空间，将产生假性动力结构，而假性吸引子对位置偏置敏感，基于此，我们有以下推测，并会在实验部分得到经验证明。



% \paragraph{Patch Embedding as Dynamics Linearization}
\begin{proposition}
The embedding method, which uses a shared linear matrix, is an integral transformation $h(t) = \int_{-\infty}^t x(s)\phi(t,s)\mathrm{d}\mu(s)$ with limited time-invariant measure $\mu$ and polynomial basis $\phi$.
\label{theo:integral}
\vspace{-1em}
\end{proposition}
Considering polynomials as universal approximators for dynamical systems \citep{bollt2021explaining}, Proposition \ref{theo:integral} indicates that mainstream embedding methods (Figure \ref{fig:embeddings}(a-c)) fundamentally projects input time series into polynomial spectral space to represent the dynamical structure, where the measure $\mu$ or weight function $\omega(s)$ is governed by patch length, $\phi$ is parameterized by the embedding matrix. 

% \begin{theorem}
%     For the full-rank embedding matrix $W$, the embedding process is a similarity transformation $W\circ f\circ{W}^{-1}$ that maintains the original dynamic properties (system eigenvalues).
% \label{theo:linear}
% \vspace{-1em}
% \end{theorem}
\begin{proposition}
    For the full-rank embedding matrix, the embedding process is a similarity transformation that maintains the original dynamic properties (system eigenvalues).
\label{theo:linear}
\vspace{-0.5em}
\end{proposition}
% Typically, the dense matrix in deep models is considered to be full rank. Theorem \ref{theo:linear} shows that the parameterized embedding process is a mere space coordinate transformation, with non-linear time series dynamics $g$ linearized by the average Jacobin value $\frac{1}{P} \sum_{i=1}^P \frac{\partial g(x)}{\partial x}$ within the data patch. 
Typically, the dense matrix in deep models is considered to be full rank. Proposition \ref{theo:linear} shows that the parameterized embedding process is a mere space coordinate transformation, with non-linear time series dynamics linearized by the average Jacobin value within the data patch. 

\begin{theorem}
A continuous function $f$ is K-Lipschitz when $\|f(x_1)-f\left(x_2\right)\|\leq K\|x_1-x_2\|$, then:

(1) The state space model with the negative diagonal matrix $\bm{A}$ and normalization layers is 1-Lipschitz.

(2) The fully connected and convolution neural network with normalization layers is 1-Lipschitz.

(3) The standard dot-product attention operation is not Lipschitz.
\vspace{-0.5em}
\label{theo:liptz}
\end{theorem}

The Lipschitz continuity restricts the changing rate of a function under random perturbations. Theorem \ref{theo:liptz} suggests that SSMs and convolution neural networks are better suited than transformers for encoding dynamical structures.  When $K=1$, the system dynamics can be considered strictly invariable. Therefore, in the following part, we can disregard the impact of the model architecture and focus exclusively on the dynamical structure changes in the embedding layer.


% \begin{proposition}
% For embedding feature space $V=span\{v^{(1)},\cdots v^{(D)}\}$, Utilizing a singular value decomposition to the model gradient $\nabla$ will reshape the 
% \label{theo:feature space}
% \end{proposition}

% 如图所示，对于正态分布初始化的嵌入矩阵V，当维度足够大时可以认为其特征空间是球形。对于传入嵌入层的梯度G，我们可以应用SVD分解GV=US，相当于嵌入层的特征空间从球形向椭球变换

\paragraph{Dynamical Feature Space} As illustrated in Figure \ref{fig:emb_duality}(a), for the embedding projection matrix $V=\operatorname{eig}(v^{1},\cdots,v^{M})$ initialized with a normal distribution, when the dimension is sufficiently large, its feature space can be considered spherical. For the gradient $\nabla$ passed into the embedding layer, we can apply the singular value decomposition (SVD) with the diagonal matrix $S=\operatorname{diag}(\sigma_1,\cdots,\sigma_M)$ and orthogonal matrix $U=(u^{1},\cdots,u^{M})$, specifically, $\nabla v^{m}=\sigma u^{m}$. 
This process can be described as the transformation of a spherical feature space (slice) into an ellipsoidal feature space.

\begin{proposition}
    The Lyapunov exponents $\lambda_m=\lim\limits_{t \rightarrow \infty} \frac{1}{t} \ln \sigma_m(t)$ of the system attractors are the mean logarithmic growth rates of the principal axes lengths of the ellipsoidal feature space. 
\label{theo:lyps}
\vspace{-0.5em}
\end{proposition}

According to Theory 3, the attractors of the system (i.e., data patterns) correspond to the ellipsoidal feature space. Scaling the embedding layer feature space using model gradients can be interpreted as an adaptive estimation of the underlying dynamical structure in time series data, and the attractor configuration is captured in the logarithm of the eigenvalues of the Oseledec matrix \citep{oseledec1968multiplicative}.  Conversely, as illustrated in Figure \ref{fig:emb_duality}(b), our proposed physics-guided embeddings (i.e., TD-Emb, HD-Emb) circumvent this process by reconstructing the dynamical trajectory using physical priors and numerical methods, directly obtaining the attractor representation through patch operations.


% \begin{lemma} Common activation functions, such as Sigmoid, Tanh, ReLU, GeLU, etc., are uniformly 1-Lipschitz continuous. Adherence to the composite rule $\|f \circ g\|_{L i p} \leq\|f\|_{L i p} \cdot\|g\|_{L i p}$, we have:

% (1) The state space model with the negative diagonal matrix $\bm{A}$ and normalization layers is 1-Lipschitz.

% (2) The fully connected and convolution neural network with normalization layers is 1-Lipschitz.

% (3) The dot-product transformer block with attention score normalization is 1-Lipschitz.
% \label{lemma:models}
% \end{lemma}

\begin{figure}
    \centering
    \vspace{-0.5em}
    \includegraphics[width=1\columnwidth]{fig/DS_scaling.png}
    \vspace{-1em}
    \caption{Illustration for (a) Parameterized embedding and (b) Physics-guided embedding technology.}
    \vspace{-1.5em}
    \label{fig:emb_duality}
\end{figure}

% Besides, the Parameterized embedding can be viewed as transforming a spherical feature space into an ellipsoidal space by the gradient to estimate the underlying dynamic structure of time series. (b) Physics-guided embedding bypasses the estimation process, deriving a dynamical system representation directly through physical prior. {\color{blue}Detailed Presentation}

\paragraph{Dynamical System Characteristics}
According to embedding theory, insufficient phase space dimensions cause dynamical structures to stack, obscuring their true shapes. Conversely, excessive dimensions expand the structure excessively, amplifying noise effects. The threshold typically equals twice the latent dynamics, and exceeding this threshold results in spurious structures. Based on this, we propose the following conjectures, which are empirically validated in Section \ref{sec:empirical exp}.

\begin{conjecture}[\textbf{Dim Scaling Law}]
\label{pro:scaling}
For parameterized embedding, as the hidden dimensions increase, the model loss will generally decrease initially and then increase, as shown in Figure \ref{fig:dim-scaling-law}.
\end{conjecture}

\begin{conjecture}
    Bidirectional non-causal modeling, whether through a transformer or SSM backbone, helps eliminate spurious dynamical structures that are sensitive to the positional inductive bias, consequently enhancing performance as empirically demonstrated in Table \ref{tab:non-casual}.
    \label{prop:bi}
\end{conjecture}

% \begin{proposition}
%     For multivariate time series within the same dynamic system, concatenating dynamic representations to form a unified system representation is recommended; for variables from different systems, the channel-independent strategy remains optimal, empirical proofed in section \ref{part:multivars}.
% \end{proposition}


